ELLA: Empowering LLMs for Interpretable, Accurate and Informative Legal Advice

Despite remarkable performance in legal consultation exhibited by legal Large Language Models(LLMs) combined with legal article retrieval components, there are still cases when the advice given is incorrect or baseless. To alleviate these problems, we propose {\bf ELLA}, a tool for {\bf E}mpowering {\bf L}LMs for interpretable, accurate, and informative {\bf L}egal {\bf A}dvice. ELLA visually presents the correlation between legal articles and LLM's response by calculating their similarities, providing users with an intuitive legal basis for the responses. Besides, based on the users' queries, ELLA retrieves relevant legal articles and displays them to users. Users can interactively select legal articles for LLM to generate more accurate responses. ELLA also retrieves relevant legal cases for user reference. Our user study shows that presenting the legal basis for the response helps users understand better. The accuracy of LLM's responses also improves when users intervene in selecting legal articles for LLM. Providing relevant legal cases also aids individuals in obtaining comprehensive information.

==> chapters/related_work.tex <==
\section{Related Work}
\subsection{LLMs in Chinese Legal domain}
LLMs have shown great potential in various domains, such as law~\cite{lai2023large} and finance~\cite{wu2023bloomberggpt, yang2023fingpt}. In the Chinese legal domain, multiple frameworks have been proposed. LawGPT~\cite{nguyen2023brief} is a series of models pre-trained on large-scale Chinese legal text and fine-tuned on legal dialogue question-and-answer datasets and judicial examination datasets. Lawyer LLaMA~\cite{lawyer-llama-report} is based on Chinese LLaMA~\cite{cui2024efficient}, learning legal knowledge through  continual training and supervised fine-tuning
task with a large-scale legal dataset. ChatLaw~\cite{cui2023chatlaw} includes ChatLaw-13B and ChatLaw-33B, finetuned based on Ziya-LLaMA-13B~\cite{yang2022zeroshot}. DICS-LawLLM~\cite{yue2023disclawllm} is based on Baichuan~\cite{yang2023baichuan} and Fuzi.mingcha~\cite{sdu_fuzi_mingcha} is based on ChatGLM~\cite{du2022glm}, which both delivers impressive performance in downstream tasks.

\subsection{Retrieval-Augment Generation}
Retrieval-Augment Generation(RAG)~\cite{lewis2021retrievalaugmented} aims at enhancing the accuracy of models with external knowledge~\cite{gao2024retrievalaugmented}. \citet{bge_embedding} propose BGE, a general embedding model that can be fine-tuned for domain-specific retrieval tasks. Due to the high computation costs for training LLMs, REPLUG~\cite{shi2023replug} and In-Context RALM~\cite{ram2023incontext} treats LLMs as a black box, propose {\it off-the-shelf} retrievers for LLMs. \citet{lin2023radit} propose RA-DIT, a lightweight fine-tuning framework that can effectively enhance LLMs with retrieval capabilities.

In the Chinese legal domain, various pre-trained models for legal case retrieval have been proposed~\cite{ma2023caseencoder, li2023sailer, su2024caseformer}. Legal domain LLMs, such as Lawyer LLaMA and ChatLaw, also provide legal article retrieval models based on BERT~\cite{devlin-etal-2019-bert} or RoBERTa~\cite{liu2019roberta}. As the legal case retrieval and article retrieval modules in our legal consultation platform are pluggable, we can flexibly deploy the aforementioned models in our system.
